Signs of Language: Embodied Sign Language Fingerspelling Acquisition from Demonstrations for Human-Robot Interaction

Learning fine-grained movements is a challenging topic in robotics, particularly in the context of robotic hands. One specific instance of this challenge is the acquisition of fingerspelling sign language in robots. In this paper, we propose an approach for learning dexterous motor imitation from video examples without additional information. To achieve this, we first build a URDF model of a robotic hand with a single actuator for each joint. We then leverage pre-trained deep vision models to extract the 3D pose of the hand from RGB videos. Next, using state-of-the-art reinforcement learning algorithms for motion imitation (namely, proximal policy optimization and soft actor-critic), we train a policy to reproduce the movement extracted from the demonstrations. We identify the optimal set of hyperparameters for imitation based on a reference motion. Finally, we demonstrate the generalizability of our approach by testing it on six different tasks, corresponding to fingerspelled letters. Our results show that our approach is able to successfully imitate these fine-grained movements without additional information, highlighting its potential for real-world applications in robotics.

==> secs/additional.tex <==
\renewcommand{\thefigure}{A\arabic{figure}}
\setcounter{figure}{0}
\renewcommand{\thetable}{A\arabic{table}}
\setcounter{table}{0}

\section{Supplementary material}

\subsection{Controller tuning}

Figure~\ref{fig:controller100} illustrates the error value for values of $k_p$ and $k_d$ in the range [0, 100], Figure~\ref{fig:controller10} for [0, 10] and Figure~\ref{fig:controller1} for [0, 1].

\begin{figure*}[ht]
    \centering
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figures/controller100}
        \caption{Max value 100}
        \label{fig:controller100}
    \end{subfigure}
    \vfill
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figures/controller10}
        \caption{Max value 10}
        \label{fig:controller10}
    \end{subfigure}
    \vfill
    \begin{subfigure}{\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figures/controller1}
        \caption{Max value 1}
        \label{fig:controller1}
    \end{subfigure}
    \caption{Exploration of different values of $k_p$ and $k_d$}
    \label{fig:controller_sweep}
\end{figure*}

\newpage

\subsection{Reinforcement learning tuning}

Table~\ref{tab:my-table} provides an alternative version of the results illustrated in Figure~\ref{fig:tuning} from the paper. The table is sorted in ascending order based on the reward. Complementarily, Figure~\ref{fig:corr} provides the correlation to the reward (i.e., last column and/or row) for each parameter. 

\begin{table}[ht]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\hline \hline
\textbf{batch\_size} &
  \textbf{gamma} &
  \textbf{learning\_rate} &
  \textbf{log\_std\_init} &
  \textbf{n\_epochs} &
  \textbf{n\_steps} &
  \textbf{ortho\_init} &
  \textbf{weight\_decay} &
  \textbf{eval/mean\_reward} \\ \hline

128 & 0.9  & 0.00001  & -2 & 10 & 1024 & false & 0.00001 & 1624.15 \\
128 & 0.9  & 0.00001  & -2 & 10 & 512  & false & 0.00001 & 1585.71 \\
128 & 0.9  & 0.00001  & -1 & 10 & 1024 & false & 0.00001 & 1531.93 \\
128 & 0.9  & 0.00001  & -2 & 10 & 512  & true  & 0.00001 & 1523.36 \\
128 & 0.9  & 0.00001  & -1 & 10 & 512  & false & 0.00001 & 1482.61 \\
128 & 0.9  & 0.00001  & -2 & 5  & 512  & true  & 0.00001 & 1471.42 \\
128 & 0.9  & 0.00001  & -2 & 5  & 512  & false & 0.00001 & 1448.38 \\
128 & 0.9  & 0.00001  & -2 & 10 & 512  & true  & 0.00001 & 1443.02 \\
128 & 0.9  & 0.00001  & -2 & 5  & 512  & true  & 0.00001 & 1422.17 \\
256 & 0.9  & 0.00001  & -2 & 5  & 1024 & true  & 0.00001 & 1413.56 \\
128 & 0.9  & 0.00003  & -1 & 10 & 1024 & false & 0.0001  & 1389.84 \\
128 & 0.95 & 0.00001  & -1 & 10 & 512  & true  & 0.00001 & 1365.09 \\
128 & 0.9  & 0.00001  & -1 & 5  & 1024 & false & 0.00001 & 1365.08 \\
128 & 0.95 & 0.00001  & -1 & 10 & 512  & false & 0.00001 & 1345.54 \\
128 & 0.9  & 0.00001  & -2 & 5  & 1024 & true  & 0.00001 & 1328.81 \\
256 & 0.95 & 0.00001  & -1 & 10 & 1024 & false & 0.00001 & 1316.15 \\
128 & 0.95 & 0.00001  & -2 & 5  & 512  & true  & 0.00001 & 1314.80 \\
128 & 0.9  & 0.00003  & -1 & 10 & 1024 & false & 0.00001 & 1300.67 \\
128 & 0.95 & 0.00001  & -2 & 10 & 512  & true  & 0.00001 & 1297.27 \\
256 & 0.9  & 0.00001  & -1 & 10 & 512  & true  & 0.00001 & 1291.71 \\
128 & 0.9  & 0.00001  & -2 & 10 & 4096 & false & 0.00001 & 1280.08 \\
128 & 0.9  & 0.00003  & -2 & 10 & 1024 & true  & 0.00001 & 1260.49 \\
256 & 0.9  & 0.00001  & -1 & 5  & 1024 & true  & 0.00001 & 1246.09 \\
256 & 0.95 & 0.00001  & -1 & 10 & 1024 & true  & 0.0001  & 1235.01 \\
128 & 0.95 & 0.00001  & -1 & 10 & 1024 & true  & 0.00001 & 1210.89 \\
256 & 0.9  & 0.00001  & -1 & 10 & 1024 & true  & 0.00001 & 1202.36 \\
256 & 0.95 & 0.00003  & -2 & 10 & 512  & true  & 0.00001 & 1194.46 \\
128 & 0.95 & 0.00003  & -1 & 10 & 1024 & false & 0.00001 & 1124.79 \\
128 & 0.95 & 0.00001  & -2 & 10 & 1024 & false & 0.00001 & 1123.54 \\
128 & 0.9  & 0.00001  & -1 & 10 & 1024 & true  & 0.00001 & 1120.74 \\
256 & 0.9  & 0.000003 & -1 & 10 & 1024 & false & 0.00001 & 1079.17 \\
128 & 0.9  & 0.000001 & -2 & 10 & 1024 & true  & 0.00001 & 1072.54 \\
128 & 0.9  & 0.000001 & -3 & 5  & 512  & true  & 0.00001 & 1057.06 \\
128 & 0.9  & 0.00003  & -2 & 3  & 4096 & true  & 0.00001 & 1044.13 \\
128 & 0.95 & 0.000001 & -2 & 5  & 1024 & true  & 0.00001 & 1042.69 \\
128 & 0.9  & 0.000003 & -1 & 5  & 1024 & false & 0.00001 & 997.65  \\
256 & 0.9  & 0.000001 & -2 & 10 & 512  & false & 0.00001 & 958.96  \\
128 & 0.95 & 0.000001 & -1 & 10 & 1024 & false & 0.00001 & 930.24  \\
512 & 0.9  & 0.000003 & -3 & 3  & 4096 & true  & 0.00001 & 929.63  \\
128 & 0.9  & 0.00003  & -1 & 10 & 512  & false & 0.00001 & 922.81  \\
256 & 0.9  & 0.00003  & -2 & 5  & 1024 & true  & 0.00001 & 915.33  \\
128 & 0.95 & 0.000001 & -1 & 10 & 512  & false & 0.00001 & 898.50  \\
128 & 0.9  & 0.000001 & -1 & 10 & 512  & true  & 0.00001 & 893.27  \\
128 & 0.95 & 0.000001 & -1 & 5  & 512  & true  & 0.00001 & 883.68  \\
128 & 0.95 & 0.00003  & -2 & 5  & 4096 & false & 0.00001 & 870.71  \\
128 & 0.9  & 0.00001  & -3 & 10 & 1024 & false & 0.00001 & 854.40 \\ \hline \hline
\end{tabular}%
}
\caption{Hyperparameters combinations and relative results for the tuning based on the reference motion}
\label{tab:my-table}
\end{table}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/correlation_matrix.png}
    \caption{Correlation matrix between hyperparameters and reward}
    \label{fig:corr}
\end{figure*}



\newpage


\subsection{Limitations}

Figure~\ref{fig:lim} illustrates the situation for the index finger when trying to perform the letter "F". We can see that, for each joint of the finger, the reference and simulated positions are very close. Hence, we concluded that the non-similarity between the imitated and reference letter "F" are due to limitations in the tracking algorithm.

\begin{figure*}[ht]
    \centering
    \begin{subfigure}{0.9\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figures/0_metacarpo.png}
        \caption{Metacarpophalangeal joint}
        \label{fig:meta}
    \end{subfigure}
    \vfill
    \begin{subfigure}{0.9\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figures/1_proximal.png}
        \caption{Proximal interphalangeal joint}
        \label{fig:proxi}
    \end{subfigure}
    \vfill
    \begin{subfigure}{0.9\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{figures/2_distal.png}
        \caption{Distal interphalangeal joint}
        \label{fig:dista}
    \end{subfigure}
    \caption{Comparison between the reference and simulated position (left) and velocity (right) of the index finger joints for the motion representing the letter "F"}
    \label{fig:lim}
\end{figure*}
